How China-Origin Vision-Language Models Move from Refusal to Reframing in State Alignment

State-aligned distortion has been documented in China-origin text-based large language models (LLMs), but whether, and in what form, it arises in multimodal systems has not been systematically examined. We construct a balanced benchmark of 200 core entries spanning ten politically sensitive topics, plus a seven-variant visual-abstraction probe, and run nine vision-language models (VLMs), seven China-origin and two non-China, across four elicitation paradigms and two prompt languages, yielding 21,708 trials. Each response is audited on six dimensions -- explicit refusal, information integrity, visual grounding, state-aligned framing, language consistency, and response length -- by two independent frontier LLM judges, validated against three human experts on a 200-trial sample. Measuring each dimension separately lets us decompose multimodal censorship into individual signals rather than a single refusal-based score; in particular, refusal and framing are measured independently, so a model can stop refusing while still reframing. We find that (i) Chinese-language prompting roughly triples the odds of state-aligned framing, within every model; (ii) China-origin models reframe more than non-China models (direction robust across judges and human raters; magnitude 1.6--3.2x); (iii) the effect is strongest in text-only political commentary (36.5%) and is gated by recognition of the depicted subject rather than pixel detail, persisting even at silhouette for iconic images; and (iv) across four Qwen generations, state-aligned framing rises while explicit refusal falls: censorship migrates from a visible act (refusal) to an invisible one (fluent reframing). We argue this shift to invisible reframing is fundamentally a problem of human-AI interaction: it removes the very signal users rely on to recognize that information has been withheld.

==> tables/t_d6_qwen_trend.tex <==
% auto-generated by analysis/compute_d6.py
\begin{table}[t]
\centering
\caption{Response length (D6) across the Qwen-VL generational series. Starred columns exclude judge-labelled refusals.}
\label{tab:d6_qwen}
\small
\begin{tabular}{llrrrrrr}
\toprule
Model & Gen & Release & n & Mean & Median & n* & Mean* \\
\midrule
Qwen2-VL-7B & 1 & 2024-08 & 2412 & 290 & 187 & 2194 & 308 \\
Qwen2.5-VL-7B & 2 & 2025-01 & 2412 & 415 & 283 & 2282 & 427 \\
Qwen3-VL-8B & 3 & 2025-09 & 2412 & 1037 & 854 & 2363 & 1053 \\
Qwen3.5-9B & 4 & 2025-11 & 2412 & 1077 & 741 & 2302 & 1120 \\
\bottomrule
\end{tabular}
\end{table}

